Prospective Learning: Learning for a Dynamic Future

In real-world applications, the distribution of the data, and our goals, evolve over time. The prevailing theoretical framework for studying machine learning, namely probably approximately correct (PAC) learning, largely ignores time. As a consequence, existing strategies to address the dynamic nature of data and goals exhibit poor real-world performance. This paper develops a theoretical framework called "Prospective Learning" that is tailored for situations when the optimal hypothesis changes over time. In PAC learning, empirical risk minimization (ERM) is known to be consistent. We develop a learner called Prospective ERM, which returns a sequence of predictors that make predictions on future data. We prove that the risk of prospective ERM converges to the Bayes risk under certain assumptions on the stochastic process generating the data. Prospective ERM, roughly speaking, incorporates time as an input in addition to the data. We show that standard ERM as done in PAC learning, without incorporating time, can result in failure to learn when distributions are dynamic. Numerical experiments illustrate that prospective ERM can learn synthetic and visual recognition problems constructed from MNIST and CIFAR-10. Code at https://github.com/neurodata/prolearn.

==> backmatter/acknowledgement.tex <==
\section*{Acknowledgements}

This paper was supported by an NSF AI Institute Planning award (\#2020312), NSF-Simons Research Collaborations on the Mathematical and Scientific Foundations of Deep Learning (MoDL), NSF-Simons Research Collaborations on Transferable, Hierarchical, Expressive, Optimal, Robust, Interpretable Networks (THEORINET, \#2031985), Microsoft Research, and DARPA. RR, RY and PC were supported by grants from the National Science Foundation (IIS-2145164, CCF-2212519), the Office of Naval Research (N00014-22-1-2255), and cloud computing credits from Amazon Web Services. The authors would like to especially thank Kathryn Vogelstein for putting up with endless meetings at the Vogelstein residence in order to make these ideas come to life.

% % Updated on 8/08/2022
% % \subsection*{References Diversity Statement}
% By our estimates (using \href{https://github.com/dalejn/cleanBib}{cleanBib}), 
% our references contain 11.47\% woman(first)/woman(last), 22.06\% man/woman, 22.06\% woman/man, and 44.41\% man/man, and 
% 11.11\% author of color (first)/author of color(last), 13.84\% white author/author of color, 14.88\% author of color/white author, and 60.17\% white author/white author.

% thank Julia Kuhl for help with the figures, and 

==> backmatter/authors.tex <==
% Define yinyang command
\newcommand{\Yinyang}[1][1]{%
    \begin{tikzpicture}[scale=#1*0.07]
      \draw[line width = #1*0.05mm,transform canvas={yshift=0.02cm}] (0,0) circle (1cm);
      \path[fill=black,transform canvas={yshift=0.02cm}] (90:1cm) arc (90:-90:0.5cm)
                        (0,0)    arc (90:270:0.5cm)
                        (0,-1cm) arc (-90:-270:1cm);
    \end{tikzpicture}}


\section*{The Future Learning Collective}

Ashwin De Silva$^{1*}$;
Rahul Ramesh$^{2*}$;
Lyle Ungar$^{2}$;
Marshall Hussain Shuler$^{1}$;
Noah J. Cowan$^{1}$;
Michael Platt$^{2}$;
Chen Li$^{1}$;
{Leyla Isik}$^{1}$;
Seung-Eon Roh$^{1}$;
Adam Charles$^{1}$;
Archana Venkataraman$^{1}$;
Brian Caffo$^{1}$;
Javier J. How$^{1}$;
Justus M Kebschull$^{1}$;
John W. Krakauer$^{1}$;
Maxim Bichuch$^{1}$;
Kaleab Alemayehu Kinfu$^{1}$;
Eva Yezerets$^{1}$;
Dinesh Jayaraman$^{2}$;
Jong M. Shin$^{1}$;
Soledad Villar$^{1}$;
Ian Phillips$^{1}$;
Carey E. Priebe$^{1}$;
Thomas Hartung$^{1}$;
Michael I. Miller$^{1}$;
% Rene Vidal$^{1}$;
Jayanta Dey$^{1}$;
Ningyuan (Teresa) Huang$^{1}$;
Eric Eaton$^{2}$;
Ralph Etienne-Cummings$^{1}$;
Elizabeth L. Ogburn$^{1}$;
Randal Burns$^{1}$;
Onyema Osuagwu$^{4}$;
Brett Mensh$^{5}$;
Alysson R. Muotri$^{6}$;
Julia Brown$^{7}$;
Chris White$^{8}$;
Weiwei Yang$^{8}$;
Andrei A. Rusu$^{9}$
{Timothy Verstynen}$^{3}$;
{Konrad P. Kording}$^{2}$; 
Pratik Chaudhari$^{2}$\textsuperscript{\Letter};
{Joshua T. Vogelstein}$^{1}$\textsuperscript{\Letter};

% 
% Kwame Kutten$^{1}$;
% Nitish Thakor$^{1}$; 
% Marilyn Albert$^{1}$;
% James J. Knierim$^{1}$;
% James B. Potash$^{1}$;
% Lena Smirnova$^{1}$; 
% Alena Savonenko$^{1}$;
% % Jeremias Sulam$^{1}$;
% Jinchong Xu$^{1}$;
% Tilak Ratnanather$^{1}$;
% Ali Geisa$^{1}$;
% Meghana Madhyastha$^{1}$;
% Tyler M. Tomita$^{1}$;
% Erik Peterson$^{3}$
% Ben Baker$^{2}$;
% Anna C. Schapiro$^{2}$;
% % 
% Leila Wehbe$^{3}$; 
% Michael J. Tarr$^{3}$; 
% % 
% Adam Kepecs$^{4}$;
% Amy Christensen$^{4}$;
% Jessica Cantlon$^{3}$;
% % 
% Bing Brunton$^{6}$;
% % 
% % 
% Gabriel Silva$^{8}$;
% Francesca Puppo$^{8}$;
% % 
% Florian Engert$^{9}$;
% % 
% Elizabeth Hillman$^{10}$;
%

\ 

\noindent
$^{1}$ Johns Hopkins University; 
$^{2}$ University of Pennsylvania;
$^{3}$ Carnegie Mellon University;
% $^{4}$ Washington University, St. Louis;
$^{4}$ Morgan State University
% $^{6}$ University of Washington;
$^{5}$ Howard Hughes Medical Institute;
$^{6}$ University of California, San Diego
% $^{9}$ Harvard University;
% $^{10}$ Columbia University;
$^{7}$ MindX;
$^{8}$ Microsoft Research
$^{9}$ DeepMind


\noindent 
$^*$ Equal contribution \\ 
\textsuperscript{\Letter} Corresponding authors:
\href{mailto:pratikac@seas.upenn.edu}{pratikac@seas.upenn.edu}, \href{mailto:jovo@progl.ai}{jovo@progl.ai}


==> backmatter/diversity.tex <==
% Updated on 8/08/2022
\section*{References Diversity Statement}
By our estimates (using \href{https://github.com/dalejn/cleanBib}{cleanBib}), 
our references contain 5.71\% woman(first)/woman(last), 11.43\% man/woman, 8.57\% woman/man, and 74.29\% man/man, and 
10.05\% author of color (first)/author of color(last), 18.07\% white author/author of color, 18.14\% author of color/white author, and 53.74\% white author/white author. 

==> backmatter/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,dsfont}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% Reference to an equation, lower-case.
\def\ineqref#1{Inequality~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}
% Reference to a definition, lower case
\def\defref#1{Definition~\ref{#1}}
% Reference to a remark, lower case
\def\remref#1{Remark~\ref{#1}}
% Reference to a conjecture, lower case
\def\conref#1{Conjecture~\ref{#1}}

\def\ceil#1{\lceil #1 \rceil}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}


\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\providecommand{\mc}[1]{\mathcal{#1}}
\providecommand{\mh}[1]{\hat{#1}}

% \newtheorem{definition}{Definition}
% \newtheorem{remark}{Remark}
% \newtheorem{conjecture}{Conjecture}


==> contents/3_old_experiments.tex <==
% !TEX root = ../NeurIPS_2024_final/neurips_2024_final.tex

\paragraph{Setup}
\begin{itemize}
\item
\textbf{Synthetic data:} Consider two binary classification tasks with one-dimensional data. The marginal distribution on the inputs is the same for both tasks, uniform over the set $[-2, -1] \cup [1, 2]$. But the ground-truth labels are flipped across them. The first classification problem assigns the label $Y=0$ to samples from $X \in [1, 2]$ and the label $Y=1$ to samples from $X \in [-2, -1]$, and the second  problem has the label assignment flipped. Let these two distributions be $U_1$ and $U_2$.
\item
\textbf{Image classification:} Both MNIST and CIFAR-10 datasets have 10 classes originally.
We create 4 probability distributions denoted by $U_1,\dots,U_4$ corresponding to images in classes $U_1 \equiv \{ 1, 2, 3, 4, 5 \}$, $U_2 \equiv \{ 4, 5, 6, 7 \}$, $U_3 \equiv \{ 6, 7, 8, 9 \}$, and $U_4 \equiv \{8, 9, 10 \}$ for both datasets.
Note that different distributions have different numbers of distinct classes, and some classes are also overlap between the distributions.
To clarify, when an input corresponding to class 4 is shown as a part of distribution $U_1$, its class index is set to 4 but if the same input is shown as a part of distribution $U_2$ then its class index is set to 1. Prospective learning problems constructed from these sets of distributions can be quite general: in existing terminology, they have covariate shift, label shift and concept drift.

We construct prospective learning problems for~\cref{eg:case2,eg:case3} using these 4 distributions.
\begin{itemize}
\item \textbf{Scenario 2}
The distribution $\P(Z_t)$ is chosen deterministically as follows:
\[
    \P(Z_t) = \begin{cases}
    U_{k+1} & \text{if } k \in \cbr{1,2,3},\\
    U_1 & \text{else}.
    \end{cases}
\]
This results in a periodic sequence of distributions $U_1, U_2, U_3, U_4, U_1, U_2 \dots$, and consequently, samples drawn from this process will be independent across time, but not identically distributed.

\item \textbf{Scenario 3}
We set up a Markov chain that transitions among the hidden states $U_1,\dots,U_4$ according to the transition matrix
\[
    \Gamma_4 = \begin{bmatrix}
                0.1 & 0.7 & 0.1 & 0.1 \\
                0.5 & 0.15 & 0.05 & 0.3 \\
                0.2 & 0.3 & 0.4 & 0.1 \\
                0.6 & 0.1 & 0.15 & 0.15 \\
            \end{bmatrix}.
\]
Marginals at different time instants of the stochastic process $\P(Z_t) = U_t$.
This is an HMM with 4 hidden states and therefore prospective learning problems corresponding to this setting fall in~\cref{eg:case3}.
We also set up a similar non-deterministic transition between the two distribution for synthetic data using the transition matrix
\[
    \Gamma_2 = \begin{bmatrix}
                0.2 & 0.8 \\
                0.6 & 0.4
            \end{bmatrix}.
\]
\end{itemize}

\item
\textbf{Reversal learning}~\citep{butter1969perseveration,schoenbaum2000changes,fellows2003ventromedial} is a concept from cognitive psychology that tests if an individual is able to make a discrimination and then reverse this choice. In our context for classification problems, reversal learning corresponds to flipping the classes of different parts of the input domain, over time. We consider two tasks\todo{PC}
\end{itemize}

In all cases, learners get $N$ samples from the distribution at each time step. We use $N=20$ and $N=10$ for synthetic data and vision tasks, respectively.

\begin{remark}[\textbf{Why we do not use existing benchmark continual learning scenarios}]
The scenarios constructed in this section resemble continual learning benchmark scenarios such as Split-MNIST or Split-CIFAR10~\citep{zenke2017continual} where data from different distributions are shown sequentially to the learner.
However, there are two major differences. First, in these existing benchmark scenarios, data distributions do not evolve in a predictable fashion. Prospective learning would not be meaningful for them. Second, existing scenarios consider a fixed time horizon. We are keen on calculating the prospective risk for much longer horizons whereby the differences between different learners are easier to discern; our experiments go for as large as 400 time steps.
\end{remark}

\paragraph{Learners.}
All learners use a multi-layer perceptron (MLP) for synthetic data problems and convolutional neural networks (CNNs), or self-attention-based architectures for problems using MNIST and CIFAR-10 data.
\begin{itemize}
\item \textbf{Time-agnostic ERM} as described in~\cref{eq:time_agnostic_erm}.
In words, this amounts to training an MLP, CNN, or the self-attention-based network on all past data. For prospective learning problems in~\cref{eg:case2,eg:case3}, this has the obvious issue that it will likely mispredict on inputs belonging to overlapping classes as the distribution switches across time between $U_1,\dots,U_4$.

\item \textbf{Prospective ERM} as described in~\cref{eq:prospective_erm} selects a hypothesis that is an infinite sequence of predictions from the hypothesis class $\HH_{i_t}$, or as described in~\cref{rem:implementing_prospective_erm} from $\HH_t$. Note that a predictor in this sequence $h_t(\cdot)$ varies with time. Therefore, an implementation of prospective ERM must use a network that takes as input some embedding of time $t$ in addition to the datum $X_t)$.
This also makes it easy to re-purpose an MLP, CNN or a self-attention-based network to return as infinite sequence of predictors, one can predict the output $Y_{t'}$ for any test datum $X_{t'}$ if the network also gets as input the time $t'$.
We encode time as a feature vector
\[
    \varphi(t) = [\sin(\w_1 t), \cos(\w_1 t), \dots, \sin(\w_d t), \cos(\w_d t)] \in \reals^{2 d},
\]
where $\w_k = 2 \pi/k$. One could also use variants of this encoding, e.g., with other sets of frequencies.
\item \textbf{(Baseline) Fine-tuning}
is a learner that fine-tunes on data from the current time $Z_t$ after building a sequence of hypotheses using all past data $Z_{< t}$.
This hypothesis is used as is for making predictions on future data.
This learner loosely resembles the popular online learning algorithm known as Follow-the-Leader~\citep{shalev2014understanding}. The two are not exactly the same because Follow-the-Leader is updated in an online fashion, while our baseline fine-tuning is not.
% This can cause forgetting which can help, or hurt, prospective risk.
\item \textbf{(Baseline) Task-agnostic continual learning}
\item
\textbf{Oracle} knows the identity of the data distribution at each time step---even for future times---though not the actual distribution itself. Using this information, the Oracle learner can build different predictors for different distributions.
This effectively amounts to solving multiple supervised learning problems.
Oracle can achieve the best in class prospective risk $\inf_{h \in \s(Z_{\leq t})} R_t(h)$ in~\cref{thm:time-aware} because it knows the identity of the data distribution at each future time $t'$.
The risk obtained by Oracle is therefore a good lower bound for the performance of the learners above, even if Oracle does not actually exploit predictable temporal patterns in the stochastic process.
Observe that the only reason Oracle predicts incorrectly on future data is that it has a finite number of samples from that distribution as a part of its training data.
\end{itemize}

\begin{remark}[\textbf{Other potential baselines}]
There are indeed many algorithms in the existing literature that the reader may think of as reasonable baselines. We have chosen a representative and relevant set here, rather than an exhaustive one. For example, online meta-learning approaches are close to fine-tuning; since our learner uses all past data to fine-tune on the current data, it is formally a superset of meta-learning algorithms~\citep{dhillon2019a}). Algorithms in the literature on time-series (i) focus on predicting future data, say, $Y_{t'}$ given past data $y_{\leq t}$ without taking covariates $X_{t'}$ or some exogenous variables $X_{\leq t}$ into account, (ii) can usually only make predictions for a pre-specified future context window~\cite{Lim2021-yx}, and (iii) work for low-dimensional signals (unlike images).
\end{remark}

See~\cref{s:app:architectures,s:app:train-eval} for more details of the architectures and the training procedure.
We use the zero-one error $\mathbf{1}\{\hat y \neq y\}$ to calculate prospective risk for all problems; all learners are trained using a standard surrogate of this objective, the cross-entropy loss.
For all experiments, for each time $t$, we calculate the prospective risk $R_t(h)$ in~\cref{eq:prospective_risk} of the hypothesis created by these learners for a particular realization of the stochastic process $z_{\leq t}$.
For each training dataset, i.e., realization of $z_{\leq t}$, the expectation in~\cref{eq:prospective_risk} is calculated over 100 realizations of the future data $Z_{> t}$. Each point in the figures is the average of three training datasets, that is, each point is an estimate of the expected prospective risk.
Unless explicitly noted, learners corresponding to different times are trained completely independently. This enables us to evaluate our learners independently on each time point, effectively increasing sample size on our evaluations.

\begin{figure}[!htpb]
    \centering
    % \includegraphics[width=0.90\linewidth]{NeuRIPS_2024/figures/case2_fig.pdf}
    \includegraphics[width=0.32\linewidth]{NeuRIPS_2024/figures/scenarios23/syn_scenario2.pdf}
    \includegraphics[width=0.32\linewidth]{NeuRIPS_2024/figures/scenarios23/mnist_scenario2.pdf}
    \includegraphics[width=0.32\linewidth]{NeuRIPS_2024/figures/scenarios23/cifar_scenario2.pdf}
    \caption{\textbf{Prospective ERM can achieve good prospective risk in~\cref{eg:case2}} for stochastic processes that consist of task sequences governed by a deterministic Markov chain. In all three types of problems, the prospective risk of Prospective learners approaches the best in class prospective risk (Oracle) with time $t$. In contrast, Retrospective-learners do not achieve a low prospective risk, it is near chance. For comparison, the chance prospective risk is 0.5 for synthetic data and 0.742 for samples from MNIST and CIFAR-10. }
    \label{fig:net_scenario2}
\end{figure}
\begin{figure}[htb]
    \centering
    % \includegraphics[width=0.5\linewidth]{NeuRIPS_2024/figures/case3_cifar10.pdf}
    \includegraphics[width=0.32\linewidth]{NeuRIPS_2024/figures/scenarios23/syn_scenario3.pdf}
    \includegraphics[width=0.32\linewidth]{NeuRIPS_2024/figures/scenarios23/mnist_scenario3.pdf}
    \includegraphics[width=0.32\linewidth]{NeuRIPS_2024/figures/scenarios23/cifar_scenario3.pdf}
    \caption{\textbf{ERM do not achieve good prospective risk in~\cref{eg:case3}}
    for stochastic processes that consist of task sequences governed by probabilistic Markov chains
    which have an invariant distribution.
    }
    \label{fig:net_scenario3}
\end{figure}

\begin{figure}[htb]
    \centering
    % \includegraphics[width=0.5\linewidth]{NeuRIPS_2024/figures/case3_cifar10.pdf}
    \includegraphics[width=0.42\linewidth]{NeuRIPS_2024/figures/scenarios23/cifar_scenario2_all.pdf}
    \includegraphics[width=0.42\linewidth]{NeuRIPS_2024/figures/scenarios23/cifar_scenario3_all.pdf}
    \label{fig:net_cifar10}
\end{figure}

\paragraph{Prospective-MLE and Prospective DNNs can learn prospectively  when data is independent but not identically distributed.}
%We first consider processes where transitions between the distributions is determined by a deterministic Markov chain (\cref{s:app:tasks}). This corresponds exactly to~\cref{eg:case2}. This corresponds to a hidden Markov model (with deterministic dynamics of the state) where the state of the HMM is the task identity, and the stochastic process is a sequence of observations from this HMM.
% As~ shows, 
Retrospective-MLP and Retrospective-CNN perform poorly in this setting (\cref{fig:net_scenario2}).
Yet, Prospective-MLE (left) and Prospective-DNNs (center and right) strongly prospectively learn.
Thus, these prospective learners can prospectively learn these stochastic processes, albeit with different sample complexities depending upon the learner.


%\vspace{-1em}

\paragraph{Prospective-MLE and Prospective-DNNs 
learn prospectively  when data is neither independent nor identically distributed.}

\todo{Yuxin: looking forward to seeing results}
% If transitions between distributions are governed by a probabilistic Markov process, then, as we show in~\cref{s:app:scenario3}, one needs to discount the future loss to make learning meaningful.
% If the Markov chain mixes and reaches an invariant distribution, then even the prospective Bayes risk can be quite high because the data is uninformative of the future, e.g., for a two-state Markov chain if the invariant distribution is $[0.5,0.5]$ then the prospective risk is at chance.


% \section{Learners}
% \label{sec:learners}

% In the above examples, we saw two explicit prospective learners based on using the Bayes plug-in principle with maximum likelihood estimators.  Here, we more formally introduce several presumptive prospective learners.
% \todo{Rubing: what do you think? did i get anything wrong?}

% \subsection{Prospective Maximum Likelihood Estimators (P-MLE).}
% %
% Let $Z_t$ be a stochastic process from some known statistical model where, for each time $t$, the maximum likelihood estimator exists. For example, at each time, $Z_t$ is Bernoulli or Gaussian stochastic periodic process, meaning the parameters changed according to a specific period $T$,  potentially in a dependent way (e.g., a first order Markov model). The Prospective Maximum Likelihood Estimator (P-MLE)  uses the MLE to obtain an estimate for  $\theta_s$ for all $s<t$. Because the P-MLE knows the statistical model (e.g., Gaussian) and the period, but not the parameters, it can then use its knowledge of the model to prospect, that is, it also yields estimates of the parameters for all future time, $\hat{\theta}_s$ for all $s \geq t$.  When we are in a discrete supervised learning setting (i.e., classification), the P-MLE selects the class with the highest estimated posterior at each time.

% In more complicated scenarios, the P-MLE might have less information about the stochastic process.  For example, it might know that the process is periodic, and that the period is bounded, but not know the period itself.  In such cases, the P-MLE estimates the parameters for each of the possible processes, and then evaluates the likelihood of each potentiall process, and selects the process with the highest likelihood.

% We run P-MLE on the four scenarios described above, and found that P-MLE converges to Prospective Bayes risk after only tens or hundreds of samples, thereby motivating the following lemma. See~\cref{s:scenarios} for details.

% \begin{lemma}
%     Prospective-MLE, as described above, in the scenarios described above, satisfies the conditions of~\cref{thm:time-aware}, and therefore, is a strong prospective learner.
% \end{lemma}

% \subsection{Prospective Deep Neural Networks (P-DNN).} We incorporate time into Deep Neural Networks (DNNs)  by computing an embedding of time and concatenating it with the input (for multilayer perceptrons, MLPs) or adding it to the output of the first convolution layer (for convolutional neural networks, CNNs), after passing it through a fully connected layer (\cref{fig:time_arch}). The time embedding contains sines and cosines for a range of frequencies, similar to the position encoding in~\citet{vaswani2017attention}. Note, however, that position encoding uses \textit{relative} position, which is bounded whereas P-DNNs use \textit{absolute} time, which is unbounded.
% Specifically, we set $\omega_i = 2\pi / i$ for $i=1, \dots, d/2$ to get a $d$-dimensional embedding of time.
% \todo{Rahul: i don't know the transformer literature well enough to know whether our autoregressive transformer is literally in the literature already, or do the `foundation models' for time series do something else? let's please clarity that.}
% %We also consider the Transformer architecture~\citep{vaswani2017attention} with the previously described time embedding. The Transformers are trained using an auto-regressive objective, where the model predicts the output at the immediate next instant $t+1$ using data $z_{\leq t}$; this is a commonly used objective for training language models~\citep{radford2019language}.

% \begin{lemma}
%     Prospective-DNN, specifically P-MLP and P-CNN, as described above, in the scenarios described above, trained using P-ERM (rather than SGD), are strong prospective learners.
% \end{lemma}


% \paragraph{Learners.} We experiment with three kinds of learners implemented using a variety of different neural architectures and hyper-parameters. \cref{s:setup} elaborates more upon this.%
% \todo{Rahul: i have no idea what the below footnote means.}
% \footnote{We should emphasize that we \emph{do not} do any continual learning for fitting the Retrospective, Prospective, prospective Transformers, or the Oracle. Even though each sample is associated with a particular time, the samples do not have to be utilized sequentially by the learner like in continual learning.
% }%



==> contents/7_neurips_checklist.tex <==
% !TEX root = ../neurips_2024_final.tex

\clearpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit.

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA).
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize}
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the list of contributions in~\cref{s:contributions} with pointers to this section from the introduction.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
    %     \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers.
    %     \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings.
    %     \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
    % \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \cref{s:discussion} discusses the limitations of our theoretical and empirical results.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper.
    %     \item The authors are encouraged to create a separate "Limitations" section in their paper.
    %     \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
    %     \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
    %     \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
    %     \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
    %     \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
    %     \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    % \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have developed substantial new theoretical results in this paper. They are discussed in~\cref{s:theory}. All mathematical claims, illustrative examples, and remarks come with elaborate proofs, both in the main paper and the Appendix.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include theoretical results.
    %     \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
    %     \item All assumptions should be clearly stated or referenced in the statement of any theorems.
    %     \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition.
    %     \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
    %     \item Theorems and Lemmas that the proof relies upon should be properly referenced.
    % \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use standard visual recognition datasets along with illustrative examples on synthetic tasks. All information to reproduce our experiments, e.g., datasets, network architectures, and training procedures, is provided in~\cref{s:setup}. All the code that was used to conduct the experiments has been made public. %\todo{Ashwin/Rahul: we need to package the code. MAKE SURE IT IS ANONYMOUS. i have heard cases where reviewers actively scout code for de-anonymizing information to reject papers (including the .git folder!!!).}
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
    %     \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable.
    %     \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
    %     \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
    %     \begin{enumerate}
    %         \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
    %         \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
    %         \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
    %         \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
    %     \end{enumerate}
    % \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the code that was used to conduct the experiments has been made public.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that paper does not include experiments requiring code.
    %     \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
    %     \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
    %     \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
    %     \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
    %     \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
    %     \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    % \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have conducted extremely thorough train/test splits, and tuned hyper-parameters manually across multiple runs. This information is provided in~\cref{s:setup}.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
    %     \item The full details can be provided either with the code, in appendix, or as supplemental material.
    % \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  For all the learning algorithms considered in every experiment in our paper, we compute empirical prospective and instantaneous risks over multiple random seeds, at $15$-$40$ different time steps. This makes our results extremely rigorous and reproducible. All experimental results in the paper come with error bars assuming a Normal distribution for the relevant quantities.
    % Every experiment in our paper is calculated across 100 test datasets (future realizations of the stochastic process), for each realization of the training dataset. For each time point, i.e., for different numbers of samples (about 12 such training datasets), three realizations of the stochastic process were used in all experiments with neural networks. This entails a total of 39 training sets, each with 100 test datasets, for each of the methods that was implemented. For synthetic data, we sampled \emph{all} binary sequences of lengths up to 20 and calculated the exact prospective risk $R_t(h)$ for every time. 
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
    %     \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
    %     \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
    %     \item The assumptions made should be given (e.g., Normally distributed errors).
    %     \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
    %     \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
    %     \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
    %     \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    % \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have conducted experiments on this problem for close to 1.5 years. In addition to the experimental results that are discussed here, there a substantial number of secondary experiments, failed attempts, that are not reported. All the experiments in this paper approximately takes $\sim 200$ GPU hours to run.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not include experiments.
    %     \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
    %     \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute.
    %     \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper).
    % \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We did not use human subjects or participants in these experiments. All our datasets are public ones that are used very commonly in the published literature, or synthetically generated. We do not anticipate societally harmful consequences of this research.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
    %     \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
    %     \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    % \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is foundational work and it is not tied to any particular application or deployment. We do not anticipate negative social impact. Down the line, when this line of research matures and it is deployed for making predictions on users, we anticipate a lot of positive social impacts, e.g., prospective learning may enable us to deploy ML models without having to retrain them as data changes over time. This improves performance because it prevents the predictions from deteriorating, but it also leads to other benefits in terms of economic and computational resources necessary to serve ML models.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that there is no societal impact of the work performed.
    %     \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
    %     \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
    %     \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
    %     \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
    %     \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    % \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We only use existing public datasets (appropriately cited in the paper) and synthetic data.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper poses no such risks.
    %     \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters.
    %     \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
    %     \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    % \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We only use existing public datasets (appropriately cited in the paper) and synthetic data. No new assets are created from this paper.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not use existing assets.
    %     \item The authors should cite the original paper that produced the code package or dataset.
    %     \item The authors should state which version of the asset is used and, if possible, include a URL.
    %     \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
    %     \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
    %     \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
    %     \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
    %     \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    % \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No assets are created in this paper.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not release new assets.
    %     \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc.
    %     \item The paper should discuss whether and how consent was obtained from people whose asset is used.
    %     \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    % \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No crowdsourcing experiments or research with human subjects.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    %     \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper.
    %     \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector.
    % \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No crowdsourcing experiments or research with human subjects.
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    %     \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.
    %     \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution.
    %     \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    % \end{itemize}

\end{enumerate}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,dsfont,amsthm,bbm, amssymb}
\usepackage{scalerel}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% Reference to an equation, lower-case.
\def\ineqref#1{Inequality~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}
% Reference to a definition, lower case
\def\Defref#1{Definition~\ref{#1}}
\def\defref#1{definition~\ref{#1}}
% Reference to a remark, lower case
\def\remref#1{Remark~\ref{#1}}
% Reference to a conjecture, lower case
\def\conref#1{Conjecture~\ref{#1}}
% Reference to a theorem, lower case
\def\theoref#1{Theorem~\ref{#1}}
% Reference to a proposition, upper case
\def\Propref#1{Proposition~\ref{#1}}
\def\propref#1{Proposition~\ref{#1}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

%\newcommand{\E}{\mathbb{E}}
%\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

%\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\providecommand{\mc}[1]{\mathcal{#1}}
\providecommand{\mh}[1]{\hat{#1}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{definition}{Definition}[section]
% \newtheorem{remark}{Remark}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{proposition}{Proposition}[section]

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}


\def \naturals {\mathbb{N}}
\def \reals {\mathbb{R}}
\def \bR {\mathbb{R}}
\def \bW {\mathbb{W}}
\def \bN {\mathbb{N}}
\def \bZ {\mathbb{Z}}
\def \bC {\mathbb{C}}

\def \rmF {\trm{F}}

\def \bb {\mathscr{b}}
\newcommand*\dd{\mathop{}\!\mathrm{d}}

\newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\agr}[1]{\left\langle#1\right\rangle}












\newcommand{\tbf}[1]{\textbf{#1}}
\newcommand{\tsf}[1]{\textsf{#1}}
\newcommand{\trm}[1]{\text{#1}}

\newcommand{\aeq}[1]{\begin{align} #1 \end{align}}
\newcommand{\aeqs}[1]{\begin{align*} #1 \end{align*}}
\newcommand{\aed}[1]{\begin{aligned} #1 \end{aligned}}
\newcommand{\beq}[1]{\begin{equation}#1\end{equation}}
\newcommand{\beqs}[1]{\begin{equation*}#1\end{equation*}}

\newcommand{\mpage}[2]{\begin{center}
\begin{minipage}{#1}#2\end{minipage}\end{center}}

% \newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
% \newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
% \newcommand{\rbr}[1]{\left(#1\right)}
% \newcommand{\sbr}[1]{\left[#1\right]}
% \newcommand{\cbr}[1]{\left\{#1\right\}}
% \newcommand{\nbr}[1]{\left\|#1\right\|}
% \newcommand{\abr}[1]{\left|#1\right|}
% \newcommand{\agr}[1]{\left\langle#1\right\rangle}
% \DeclarePairedDelimiter{\norm}{\lVert}{\rVert}

\newcommand{\indep}
{\perp\!\!\!\perp}
% {\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\la}{\ \leftarrow\ }
% \newcommand{\ra}{\rightarrow}
%\newcommand{\from}{\la}
\providecommand\f[2]{\ensuremath \frac{#1}{#2}}

\DeclareMathOperator{\given}{\, \vert\ }
%\DeclareMathOperator*{\argmin}{\text{argmin}}
%\DeclareMathOperator*{\argmax}{\text{argmax}}
\DeclareMathOperator{\sign}{\text{sign}}
\DeclareMathOperator{\logdet}{\text{logdet}}
\DeclareMathOperator{\diag}{\text{diag}}
\let\P\relax
\DeclareMathOperator{\P}{\mathbb{P}}
\DeclareMathOperator*{\E}{\mathbb{E}}
\DeclareMathOperator*{\Var}{\text{Var}}
\DeclareMathOperator*{\cov}{\text{Cov}}
% \DeclarePairedDelimiter\ceil{\lceil}{\rceil}
% \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\providecommand{\ones}{\mathds{1}}
\providecommand{\ind}[1]{{\bf 1}_{\cbr{#1}}}
\providecommand{\nnot}[1]{\overline{#1}}
\providecommand{\oor}{\vee}
\providecommand{\aand}{\wedge}
\renewcommand{\implies}{\Rightarrow}

\newcommand{\der}[2]{\f{\trm{d}\; #1}{\trm{d}\; #2} }
\newcommand{\pder}[2]{\f{\partial #1}{\partial #2} }
\newcommand{\fder}[2]{\f{\d #1}{\d #2} }
\newcommand{\what}[1]{\widehat{#1}}

\def \d {\delta}
\def \s {\sigma}
\def \w {\omega}
\def \r {\rho}
\def \t {\tau}
\def \th {\theta}
\def \a {\alpha}
\def \b {\beta}
\def \p {\phi}
\def \e {\epsilon}
\def \g {\gamma}
\def \z {\zeta}
\def \l {\lambda}
\def \k {\kappa}

\def \D {\Delta}
\def \G {\Gamma}
\def \L {\Lambda}
\def \S {\Sigma}
\def \Th {\Theta}
\def \Om {\Omega}
\def \tOm {\widetilde{\Om}}

\def \TT {\mathcal{T}}
\def \CC {\mathcal{C}}
\def \XX {\mathcal{X}}
\def \YY {\mathcal{Y}}
\def \LL {\mathcal{L}}
\def \QQ {\mathcal{Q}}
\def \DD {\mathcal{D}}
\def \FF {\mathcal{F}}
\def \HH {\mathcal{H}}
\def \GG {\mathcal{G}}
\def \OO {\mathcal{O}}
\def \tOO {\widetilde{\mathcal{O}}}
\def \BB {\mathcal{B}}
\def \PP {\mathcal{P}}
\def \EE {\mathcal{E}}

\def \naturals {\mathbb{N}}
\def \reals {\mathbb{R}}
\def \bR {\mathbb{R}}
\def \bW {\mathbb{W}}
\def \bN {\mathbb{N}}
\def \bZ {\mathbb{Z}}
\def \bC {\mathbb{C}}

\def \rmF {\trm{F}}

\def \bb {\mathscr{b}}



% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
\theoremstyle{definition}
% \newtheorem{definition}{Definition}
\newtheorem{example}{Example}
% \newtheorem{remark}{Remark}
\newtheorem{scenario}{Scenario}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \newcommand{\iid}{\overset{iid}{\sim}}

\Crefname{example}{Example}{Examples}
\Crefname{scenario}{Scenario}{Scenarios}

\providecommand{\mc}[1]{\mathcal{#1}}

\newcommand{\done}{\ding{51}}%
% \renewcommand{\cross}{\ding{55}}%
\newcommand{\writing}{\ding{46}}%
\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=\cross}

\makeatletter
\newcommand{\InlineColorBox}[2]{%
  \Colorbox{#1}{#2}%
}
\makeatother

\newcommand{\rahul}{\InlineColorBox{orange!30}{rahul}~}
\newcommand{\ashwin}{\InlineColorBox{black!5!cyan!30}{ashwin}~}
\newcommand{\rubing}{\InlineColorBox{black!30!green!30}{rubing}~}

% citations make colored
\hypersetup{
    colorlinks=true,
    linkcolor=cyan!70!black,
    filecolor=magenta,      
    urlcolor=cyan,
    citecolor=cyan!60!black,
}

% \newcommand{\tbf}[1]{\textbf{#1}}
% \newcommand{\tsf}[1]{\textsf{#1}}
% \newcommand{\trm}[1]{\text{#1}}

% \newcommand{\aeq}[1]{\begin{align} #1 \end{align}}
% \newcommand{\aeqs}[1]{\begin{align*} #1 \end{align*}}
% \newcommand{\aed}[1]{\begin{aligned} #1 \end{aligned}}
% \newcommand{\beq}[1]{\begin{equation}#1\end{equation}}
% \newcommand{\beqs}[1]{\begin{equation*}#1\end{equation*}}

% \newcommand{\mpage}[2]{\begin{center}
% \begin{minipage}{#1}#2\end{minipage}\end{center}}

% \newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
% \newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
% \newcommand{\rbr}[1]{\left(#1\right)}
% \newcommand{\sbr}[1]{\left[#1\right]}
% \newcommand{\cbr}[1]{\left\{#1\right\}}
% \newcommand{\nbr}[1]{\left\|#1\right\|}
% \newcommand{\abr}[1]{\left|#1\right|}
% \newcommand{\agr}[1]{\left\langle#1\right\rangle}
% % \DeclarePairedDelimiter{\norm}{\lVert}{\rVert}

% \newcommand{\indep}
% {\perp\!\!\!\perp}
% % {\protect\mathpalette{\protect\independenT}{\perp}}
% \def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

% \newcommand{\la}{\ \leftarrow\ }
% \newcommand{\ra}{\rightarrow}
% %\newcommand{\from}{\la}
% \providecommand\f[2]{\ensuremath \frac{#1}{#2}}

% \DeclareMathOperator{\given}{\, \vert\ }
% %\DeclareMathOperator*{\argmin}{\text{argmin}}
% %\DeclareMathOperator*{\argmax}{\text{argmax}}
% \DeclareMathOperator{\sign}{\text{sign}}
% \DeclareMathOperator{\logdet}{\text{logdet}}
% \DeclareMathOperator{\diag}{\text{diag}}
% \let\P\relax
% \DeclareMathOperator{\P}{\mathbb{P}}
% \DeclareMathOperator*{\E}{\mathbb{E}}
% \DeclareMathOperator*{\Var}{\text{Var}}
% \DeclareMathOperator*{\cov}{\text{Cov}}
% % \DeclarePairedDelimiter\ceil{\lceil}{\rceil}
% % \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% \providecommand{\ones}{\mathds{1}}
% \providecommand{\ind}[1]{{\bf 1}_{\cbr{#1}}}
% \providecommand{\nnot}[1]{\overline{#1}}
% \providecommand{\oor}{\vee}
% \providecommand{\aand}{\wedge}
% \renewcommand{\implies}{\Rightarrow}

% \newcommand{\der}[2]{\f{\trm{d}\; #1}{\trm{d}\; #2} }
% \newcommand{\pder}[2]{\f{\partial #1}{\partial #2} }
% \newcommand{\fder}[2]{\f{\d #1}{\d #2} }
% \newcommand{\what}[1]{\widehat{#1}}

\def \d {\delta}
\def \s {\sigma}
\def \w {\omega}
\def \r {\rho}
\def \t {\tau}
\def \th {\theta}
\def \a {\alpha}
\def \b {\beta}
\def \p {\phi}
\def \e {\epsilon}
\def \g {\gamma}
\def \z {\zeta}
\def \l {\lambda}
\def \k {\kappa}

\def \D {\Delta}
\def \G {\Gamma}
\def \L {\Lambda}
\def \S {\Sigma}
\def \Th {\Theta}
\def \Om {\Omega}
\def \tOm {\widetilde{\Om}}

\def \TT {\mathcal{T}}
\def \CC {\mathcal{C}}
\def \XX {\mathcal{X}}
\def \YY {\mathcal{Y}}
\def \LL {\mathcal{L}}
\def \QQ {\mathcal{Q}}
\def \DD {\mathcal{D}}
\def \FF {\mathcal{F}}
\def \HH {\mathcal{H}}
\def \GG {\mathcal{G}}
\def \OO {\mathcal{O}}
\def \tOO {\widetilde{\mathcal{O}}}
\def \BB {\mathcal{B}}
\def \PP {\mathcal{P}}
\def \EE {\mathcal{E}}

\def \naturals {\mathbb{N}}
\def \reals {\mathbb{R}}
\def \bR {\mathbb{R}}
\def \bW {\mathbb{W}}
\def \bN {\mathbb{N}}
\def \bZ {\mathbb{Z}}
\def \bC {\mathbb{C}}

\def \rmF {\trm{F}}

\def \bb {\mathscr{b}}
